Item Tagging for Information Retrieval: A Tripartite Graph Neural Network based Approach

Tagging has been recognized as a successful practice to boost relevance matching for information retrieval (IR), especially when items lack rich textual descriptions. A lot of research has been done for either multi-label text categorization or image annotation. However, there is a lack of published work that targets at item tagging specifically for IR. Directly applying a traditional multi-label classification model for item tagging is sub-optimal, due to the ignorance of unique characteristics in IR. In this work, we propose to formulate item tagging as a link prediction problem between item nodes and tag nodes. To enrich the representation of items, we leverage the query logs available in IR tasks, and construct a query-item-tag tripartite graph. This formulation results in a TagGNN model that utilizes heterogeneous graph neural networks with multiple types of nodes and edges. Different from previous research, we also optimize both full tag prediction and partial tag completion cases in a unified framework via a primary-dual loss mechanism. Experimental results on both open and industrial datasets show that our TagGNN approach outperforms the state-of-the-art multi-label classification approaches.

==> sections/2_background.tex <==

\section{Background}\label{sec_background}
In this section, we briefly introduce the background of CTR prediction and knowledge distillation. %, which is a core task in online advertising, Web search, and recommender systems. 

\subsection{Item Tagging}\label{sec:ctr}
%The goal of CTR prediction is to predict the probability a user will click a candidate item. %Hence, it can be naturally modelled as a binary classification problem.  For applications with a large user base, even a small improvement in prediction accuracy can potentially lead to a large increase of the overall revenue. For example, an absolute improvement of 1\textperthousand ~in AUC (or logloss) is considered as practically significant in real CTR prediction problems~\cite{DCN,autoint}. However, making accurate CTR prediction remains a great challenge. In contrast to other data types, such as images and texts, data in CTR prediction problems are usually of large scale and high sparsity, involving categorical features of multiple fields (e.g., billions of samples with millions of features in app recommendation of Google Play~\cite{WideDeep}).



\subsection{Graph Neural Networks}\label{sec:ctr}

With the success of deep learning, CTR prediction models have been evolved from traditional linear models (e.g. LR~\cite{LR}, FTRL~\cite{FTRL}), factorization machines (e.g., FM~\cite{FM}, FFM~\cite{FFM}), to deep neural networks (e.g., Wide\&Deep~\cite{WideDeep}, DeepFM~\cite{DeepFM}). Compared with shallow models such as LR and FM, deep models are powerful in capturing sophisticated high-order feature interactions with nonlinear activation functions and thus lead to better performance. %Theoretically, a vanilla DNN (i.e., MLP) is able to learn arbitrarily complex feature interactions. However, this DNN model is found to be prone to overfitting in practice due to the fact that useful interactions are extremely sparse compared with the entire combination space of features. To improve over the vanilla DNN, many improvements have been made recently. 

Formally, the objective of CTR prediction is to learn a model that maps input features $x$ to an estimated click probability $\hat{y}\in[0,1]$, 
We define $\hat{y}=\sigma(\phi(x))$, where $\phi(x)$ is the model function that outputs the logit (un-normalized log probability value) given $x$ and $\sigma(\cdot)$ is the sigmoid function. In the following, we briefly describe four of the most representative models. While we focus only on illustrating the core ideas of these models, interested readers may refer to their papers for more details.


==> sections/4_experiment.tex <==
% Significance Test. We repeat the experiments 10 times
%for FGCNN and the best baseline model. The two-tailed
%pairwise t-test is performed to detect significant differences
%between FGCNN and the best baseline model.

% FGCNN achieves the best performance among all
% the models on the three evaluated datasets. It is significantly
% better than the best baseline models with 0.05%, 0.14% and
% 0.13% improvements in AUC (0.09%, 0.24% and 0.79% in
% log loss) on Criteo, Avazu and Company datasets, which
% demonstrates the effectiveness of FGCNN. In fact, a small
% improvement in offline AUC is likely to lead to a significant
% increase in online CTR. As reported in [8], compared with
% LR, Wide & Deep improves offline AUC by 0.275% and the
% improvement of online CTR is 3.9%. The daily turnover of
% Company’s App Store is millions of dollars. Therefore, even
% a few percents lift in CTR brings extra millions of dollars
% each year.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%https://www.tablesgenerator.com/latex_tables
% \begin{table*}[]
% \centering
% \small
% \caption{}
% \label{tab:benchmark}
% \begin{tabular}{cllllllccllllllcl}
% \hline
% \multicolumn{1}{c|}{\multirow{2}{*}{}} & \multicolumn{8}{c|}{Criteo} & \multicolumn{8}{c|}{Avazu} \\ \cline{2-7} \cline{10-15}
% \multicolumn{1}{c|}{} & \multicolumn{2}{c|}{Original} & \multicolumn{2}{c|}{Reproduced} & \multicolumn{2}{c|}{Retuned} & \multirow{2}{*}{\#Runs} & \multicolumn{1}{c|}{Time/Epoch} & \multicolumn{2}{c|}{Original} & \multicolumn{2}{c|}{Reproduced} & \multicolumn{2}{c|}{Retuned} & \multicolumn{1}{l}{\multirow{2}{*}{\#Runs}} & \multicolumn{1}{c}{Time/Epoch} \\ \cline{1-7} \cline{10-15}
% \multicolumn{1}{c|}{Model} & \multicolumn{1}{c}{Logloss} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c}{Logloss} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c}{Logloss} & \multicolumn{1}{c}{AUC} &  & \multicolumn{1}{c|}{(Mins)} & \multicolumn{1}{c}{Logloss} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c}{Logloss} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c}{Logloss} & \multicolumn{1}{c}{AUC} & \multicolumn{1}{l}{} & \multicolumn{1}{c}{(Mins)} \\ \cline{1-7} \cline{9-15} \cline{17-17} 
% \multicolumn{1}{c|}{LR} & \multicolumn{1}{c}{—} & \multicolumn{1}{c|}{—} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{0.45651} & \multicolumn{1}{c}{0.79363} & 12 & \multicolumn{1}{c|}{xx} & \multicolumn{1}{c}{—} & \multicolumn{1}{c|}{—} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{0.37991} & \multicolumn{1}{c}{0.78048} & 90 & \multicolumn{1}{c}{180} \\
% \multicolumn{1}{c|}{FM} & \multicolumn{1}{c}{—} & \multicolumn{1}{c|}{—} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{0.44432} & \multicolumn{1}{c}{0.80804} & 20 & \multicolumn{1}{c|}{xx} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{0.37363} & \multicolumn{1}{c}{0.79079} & 187 & \multicolumn{1}{c}{} \\
% \multicolumn{1}{c|}{CCPM} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{0.44467} & \multicolumn{1}{c}{0.80692} & 24 & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{0.37183} & \multicolumn{1}{c}{0.79355} & 24 &  \\
% HOFM &  &  &  &  &  &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  &  &  & \multicolumn{1}{l}{} &  \\
% \multicolumn{1}{c|}{FFM} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{0.44091} & \multicolumn{1}{c}{0.81109} & 20 & \multicolumn{1}{c|}{xx} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{0.37114} & \multicolumn{1}{c}{0.79484} & 32 &  \\
% DNN & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{0.44071} & \multicolumn{1}{c}{0.81120} & 64 & \multicolumn{1}{l}{} &  &  &  &  & 0.37048 & 0.79583 & 252 &  \\
% \multicolumn{1}{l}{WideDeep} &  &  &  &  & 0.43916 & 0.81261 & 64 & \multicolumn{1}{l}{} &  &  &  &  & 0.37034 & 0.79575 & 52 &  \\
% IPNN &  &  &  &  & 0.43909 & 0.81273 & 64 & \multicolumn{1}{l}{} &  &  &  &  & 0.36839 & 0.79885 & 36 &  \\
% \multicolumn{1}{l}{DeepCross} &  &  &  &  & 0.43804 & 0.81395 & 138 & \multicolumn{1}{l}{} &  &  &  &  & 0.37002 & 0.79620 & 45 &  \\
% NFM &  &  &  &  & 0.44431 & 0.80718 & 64 & \multicolumn{1}{l}{} &  &  &  &  & 0.37146 & 0.79399 & 54 &  \\
% \multicolumn{1}{c|}{AFM} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{0.44430} & \multicolumn{1}{c}{0.80732} & 10 & \multicolumn{1}{c|}{xx} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{0.37809} & \multicolumn{1}{c}{0.78403} & 67 &  \\
% DeepFM &  &  &  &  & 0.43779 & 0.81407 & 128 & \multicolumn{1}{l}{} &  &  &  &  & 0.37002 & 0.79645 & 176 &  \\
% DCN &  &  &  &  & \multicolumn{1}{c}{0.43783} & 0.81407 & 544 & \multicolumn{1}{c|}{xx} &  &  &  &  & 0.36993 & 0.79652 & 496 &  \\
% \multicolumn{1}{c|}{FwFM} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} & 0.44189 & 0.80991 & 20 & \multicolumn{1}{c|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} & 0.37277 & 0.79197 & 12 &  \\
% \multicolumn{1}{c|}{xDeepFM} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} & 0.43776 & 0.81426 & 156 & \multicolumn{1}{c|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} & 0.36987 & 0.79650 & 72 &  \\
% \multicolumn{1}{c|}{HFM+} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  &  &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} & 0.36923 & 0.79787 & 92 &  \\
% \multicolumn{1}{c|}{FGCNN} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} & 0.43968 & 0.81216 & xx & \multicolumn{1}{c|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} & 0.36961 & 0.79705 & 84 &  \\
% \multicolumn{1}{c|}{AutoInt+} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} & 0.44148 & 0.81018 & 72 & \multicolumn{1}{c|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} & 0.37031 & 0.79587 & 75 &  \\
% \multicolumn{1}{c|}{FiGNN} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} & 0.43781 & 0.81410 & 40 & \multicolumn{1}{c|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} & 0.37113 & 0.79442 & 64 &  \\
% \multicolumn{1}{c|}{ONN} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} & 0.43805 & 0.81415 & 108 & \multicolumn{1}{c|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} & 0.36767 & 0.80012 & \multicolumn{1}{l}{120} &  \\
% \multicolumn{1}{c|}{FiBiNET} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} & 0.43859 & 0.81328 & 60 & \multicolumn{1}{c|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} & 0.36714 & 0.80088 & \multicolumn{1}{l}{54} &  \\
% LorentzFM &  &  &  &  &  &  &  & \multicolumn{1}{l}{} &  &  &  &  & 0.37417 & 0.79122 & \multicolumn{1}{l}{9} &  \\
% \multicolumn{1}{c|}{AFN+} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} & 0.43865 & 0.81336 & 114 & \multicolumn{1}{c|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} & 0.37061 & 0.79561 & \multicolumn{1}{l}{190} &  \\
% \multicolumn{1}{c|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  &  &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  &  & \multicolumn{1}{l}{} &  \\ \cline{1-7} \cline{10-15}
% \end{tabular}
% \end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %https://www.tablesgenerator.com/latex_tables
% \begin{table*}[]
% \centering
% \small
% \caption{FuxiCTR Benchmarking Results}
% \begin{tabular}{c|c|cc|rr|c|c|cc|rrcc}
% \hline
% \multicolumn{2}{c|}{\multirow{2}{*}{\textbf{}}} & \multicolumn{6}{c|}{\textbf{Criteo}} & \multicolumn{6}{c|}{\textbf{Avazu}} \\ \cline{3-14} 
% \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{Best Reported} & \multicolumn{4}{c|}{Retuned} & \multicolumn{2}{c|}{Best Reported} & \multicolumn{4}{c}{Retuned} \\ \hline
% Year & Model & Logloss & AUC & \multicolumn{1}{c}{Logloss} & \multicolumn{1}{c|}{AUC} & \#Params & \#Runs & Logloss & AUC & \multicolumn{1}{c}{Logloss} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{\#Params} & \#Runs \\ \hline
% — & LR & {\ul 0.4474} & 0.7858 & 0.45651 & 0.79363 &  & 12 & 0.3868 & 0.7676 & 0.37991 & \multicolumn{1}{r|}{0.78048} & \multicolumn{1}{c|}{} & 90 \\
%  &  &  &  & ±0.00003 & ±0.00003 &  &  &  &  & ±0.00001 & \multicolumn{1}{r|}{±0.00006} & \multicolumn{1}{c|}{} &  \\
% 2010 & FM & 0.4464 & 0.7933 & 0.44432 & 0.80804 &  & 20 & 0.3740 & 0.7793 & 0.37363 & \multicolumn{1}{r|}{0.79079} & \multicolumn{1}{c|}{} & 187 \\
%  &  &  &  & ±0.00010 & ±0.00015 &  &  &  &  & ±0.00011 & \multicolumn{1}{r|}{±0.00018} & \multicolumn{1}{c|}{} &  \\
% 2015 & CCPM & — & — & 0.44467 & 0.80692 &  & 24 & 0.3800 & 0.7812 & 0.37183 & \multicolumn{1}{r|}{0.79355} & \multicolumn{1}{c|}{} & 24 \\
% \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00012 & ±0.00011 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00045 & \multicolumn{1}{r|}{±0.00072} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} \\
% 2016 & HOFM & 0.4508 & 0.8005 &  &  &  &  & 0.3756 & 0.7701 & 0.37351 & \multicolumn{1}{r|}{0.79131} & \multicolumn{1}{c|}{} & 19 \\
% \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} &  &  & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00011 & \multicolumn{1}{r|}{±0.00029} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} \\
% 2016 & FFM & 0.4525 & 0.8001 & 0.44091 & 0.81109 &  & 20 & 0.3781 & 0.7831 & 0.37114 & \multicolumn{1}{r|}{0.79484} & \multicolumn{1}{c|}{} & 32 \\
% \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00031 & ±0.00031 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00022 & \multicolumn{1}{r|}{±0.00044} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} \\
% 2016 & DNN & 0.4491 & 0.7993 & 0.44071 & 0.81120 &  & 64 & — & — & 0.37048 & \multicolumn{1}{r|}{0.79583} & \multicolumn{1}{c|}{} & 252 \\
% \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00006 & ±0.00009 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00009 & \multicolumn{1}{r|}{±0.00008} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} \\
% 2016 & WideDeep & 0.4453 & 0.8062 & 0.43916 & 0.81261 &  & 64 & 0.3744 & 0.7749 & 0.37034 & \multicolumn{1}{r|}{0.79575} & \multicolumn{1}{c|}{} & 52 \\
% \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00013 & ±0.00010 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00004 & \multicolumn{1}{r|}{±0.00006} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} \\
% 2016 & IPNN & 0.4532 & 0.8038 & 0.43884 & 0.81324 &  & 38 & 0.3737 & 0.7868 & 0.36839 & \multicolumn{1}{r|}{0.79885} & \multicolumn{1}{c|}{} & 36 \\
% \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00008 & ±0.00006 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00005 & \multicolumn{1}{r|}{±0.00007} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} \\
% 2016 & DeepCross & 0.4425 & 0.8009 & 0.43804 & 0.81395 &  & 138 & 0.3889 & 0.7643 & 0.37002 & \multicolumn{1}{r|}{0.79620} & \multicolumn{1}{c|}{} & 45 \\
% \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00059 & ±0.00060 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00008 & \multicolumn{1}{r|}{±0.00010} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} \\
% 2017 & NFM & 0.4537 & 0.7968 & 0.44431 & 0.80718 &  & 64 & 0.3761 & 0.7708 & 0.37146 & \multicolumn{1}{r|}{0.79399} & \multicolumn{1}{c|}{} & 54 \\
% \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00003 & ±0.00005 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00005 & \multicolumn{1}{r|}{±0.00006} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} \\
% 2017 & AFM & 0.4541 & 0.7965 & 0.44430 & 0.80732 &  & 10 & 0.3766 & 0.7740 & 0.37809 & \multicolumn{1}{r|}{0.78403} & \multicolumn{1}{c|}{} & 67 \\
% \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00074 & ±0.00080 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00067 & \multicolumn{1}{r|}{±0.00129} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} \\
% 2017 & DeepFM & 0.4445 & 0.8085 & 0.43779 & 0.81407 &  & 128 & 0.3742 & 0.7836 & 0.37002 & \multicolumn{1}{r|}{0.79645} & \multicolumn{1}{c|}{} & 176 \\
% \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00005 & ±0.00007 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00005 & \multicolumn{1}{r|}{±0.00011} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} \\
% 2017 & DCN & 0.4419 & 0.8067 & 0.43783 & 0.81407 &  & 544 & 0.3721 & 0.7681 & 0.36993 & \multicolumn{1}{r|}{0.79652} & \multicolumn{1}{c|}{} & 496 \\
% \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00017 & ±0.00012 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00013 & \multicolumn{1}{r|}{±0.00011} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} \\
% 2018 & FwFM & — & — & 0.44189 & 0.80985 &  & 14 & 0.3988 & 0.7406 & 0.37240 & \multicolumn{1}{r|}{0.79253} & \multicolumn{1}{c|}{} & 15 \\
% \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00009 & ±0.00010 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00024 & \multicolumn{1}{r|}{±0.00035} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} \\
% 2018 & xDeepFM & 0.4418 & 0.8091 & \textbf{0.43776} & \textbf{0.81426} &  & 156 & 0.3737 & 0.7855 & 0.36987 & \multicolumn{1}{r|}{0.79650} & \multicolumn{1}{c|}{} & 72 \\
% \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00019 & ±0.00020 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00013 & \multicolumn{1}{r|}{±0.00024} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} \\
% 2019 & HFM+ & — & — & 0.43911 & 0.81271 &  & 74 & — & — & 0.36923 & \multicolumn{1}{r|}{0.79787} & \multicolumn{1}{c|}{} & 92 \\
% \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} &  &  & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00004 & \multicolumn{1}{r|}{±0.00003} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} \\
% 2019 & FGCNN & — & — & 0.43814 & 0.81418 &  & 87 & 0.3746 & 0.7883 & 0.36961 & \multicolumn{1}{r|}{0.79705} & \multicolumn{1}{c|}{} & 84 \\
% \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00021 & ±0.00031 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00018 & \multicolumn{1}{r|}{±0.00027} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} \\
% 2019 & AutoInt+ & 0.4434 & 0.8083 & 0.44148 & 0.81018 &  & 72 & 0.3811 & 0.7774 & 0.37031 & \multicolumn{1}{r|}{0.79587} & \multicolumn{1}{c|}{} & 75 \\
% \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00002 & ±0.00004 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00017 & \multicolumn{1}{r|}{±0.00007} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} \\
% 2019 & FiGNN & 0.4411 & 0.8082 & 0.43781 & 0.81410 &  & 40 & 0.3817 & {\ul 0.8120} & 0.37113 & \multicolumn{1}{r|}{0.79442} & \multicolumn{1}{c|}{} & 64 \\
% \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00010 & ±0.00007 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00009 & \multicolumn{1}{r|}{±0.00014} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} \\
% 2019 & ONN & {\ul 0.43577} & 0.8123 & 0.43805 & 0.81415 &  & 108 & 0.3945 & 0.7513 & 0.36767 & \multicolumn{1}{r|}{0.80012} & \multicolumn{1}{c|}{} & 120 \\
% \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00016 & ±0.00027 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00041 & \multicolumn{1}{r|}{±0.00009} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} \\
% 2019 & FiBiNET & 0.4423 & 0.8103 & 0.43857 & 0.81335 &  & 78 & 0.3786 & 0.7832 & \textbf{0.36714} & \multicolumn{1}{r|}{\textbf{0.80088}} & \multicolumn{1}{c|}{} & 54 \\
% \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00021 & ±0.00008 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00024 & \multicolumn{1}{r|}{±0.00030} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} \\
% 2020 & LorentzFM & — & — & 0.44132 & 0.81055 &  & 8 & 0.3828 & 0.7775 & 0.37417 & \multicolumn{1}{r|}{0.79122} & \multicolumn{1}{c|}{} & 9 \\
% \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} &  &  & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00092 & \multicolumn{1}{r|}{±0.00199} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} \\
% 2020 & AFN+ & 0.4451 & 0.8074 & 0.43865 & 0.81336 &  & 114 & 0.3718 & 0.7555 & 0.37061 & \multicolumn{1}{r|}{0.79561} & \multicolumn{1}{c|}{} & 190 \\
% \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00015 & ±0.00007 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & ±0.00017 & \multicolumn{1}{r|}{±0.00029} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} \\ \hline
% \end{tabular}
% \end{table*}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%https://www.tablesgenerator.com/latex_tables
\begin{table*}[]
\centering
\small
\caption{FuxiCTR Benchmarking Results}
\begin{tabular}{ccccccccccc}
\hline
\multicolumn{11}{c}{\textbf{Criteo}} \\ \hline
\multicolumn{2}{c|}{\textbf{}} & \multicolumn{2}{c|}{Best Reported} & \multicolumn{2}{c|}{Reproduced} & \multicolumn{4}{c|}{Retuned} & Training \\ \hline
\multicolumn{1}{c|}{Year} & \multicolumn{1}{c|}{Model} & Logloss & \multicolumn{1}{c|}{AUC} & Logloss & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{Logloss} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{\#Params} & \multicolumn{1}{c|}{\#Runs} & Time x Epochs \\ \hline
\multicolumn{1}{c|}{—} & \multicolumn{1}{c|}{LR} & {\ul 0.4474} & \multicolumn{1}{c|}{0.7858} & 0.45651 & \multicolumn{1}{c|}{0.45651} & \multicolumn{1}{c|}{0.45651 ± 0.00003} & \multicolumn{1}{c|}{0.79363 ± 0.00003} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{12} & 7m x 12 \\
\multicolumn{1}{c|}{2010} & \multicolumn{1}{c|}{FM} & 0.4464 & \multicolumn{1}{c|}{0.7933} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.44432 ± 0.00010} & \multicolumn{1}{c|}{0.80804 ± 0.00015} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{20} & 18mx5 \\
\multicolumn{1}{c|}{2015} & \multicolumn{1}{c|}{CCPM} & — & \multicolumn{1}{c|}{—} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.44467 ± 0.00012} & \multicolumn{1}{c|}{0.80692 ± 0.00011} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{24} & 2h33m x 1 \\
\multicolumn{1}{c|}{2016} & \multicolumn{1}{c|}{HOFM} & 0.4508 & \multicolumn{1}{c|}{0.8005} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  \\
\multicolumn{1}{c|}{2016} & \multicolumn{1}{c|}{FFM} & 0.4525 & \multicolumn{1}{c|}{0.8001} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.44091 ± 0.00031} & \multicolumn{1}{c|}{0.81109 ± 0.00031} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{20} & 3h59m x 5 \\
\multicolumn{1}{c|}{2016} & \multicolumn{1}{c|}{DNN} & 0.4491 & \multicolumn{1}{c|}{0.7993} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.44071 ± 0.00006} & \multicolumn{1}{c|}{0.81120 ± 0.00009} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{64} & 13m x 2 \\
\multicolumn{1}{c|}{2016} & \multicolumn{1}{c|}{WideDeep} & 0.4453 & \multicolumn{1}{c|}{0.8062} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.43916 ± 0.00013} & \multicolumn{1}{c|}{0.81261 ± 0.00010} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{64} & 18m \\
\multicolumn{1}{c|}{2016} & \multicolumn{1}{c|}{IPNN} & 0.4532 & \multicolumn{1}{c|}{0.8038} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.43884 ± 0.00008} & \multicolumn{1}{c|}{0.81324 ± 0.00006} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{38} & 32m x 2 \\
\multicolumn{1}{c|}{2016} & \multicolumn{1}{c|}{DeepCross} & 0.4425 & \multicolumn{1}{c|}{0.8009} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.43804 ± 0.00059} & \multicolumn{1}{c|}{0.81395 ± 0.00060} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{138} & 26m x 3 \\
\multicolumn{1}{c|}{2017} & \multicolumn{1}{c|}{NFM} & 0.4537 & \multicolumn{1}{c|}{0.7968} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.44431 ± 0.00003} & \multicolumn{1}{c|}{0.80718 ± 0.00005} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{64} & 18m x 2 \\
\multicolumn{1}{c|}{2017} & \multicolumn{1}{c|}{AFM} & 0.4541 & \multicolumn{1}{c|}{0.7965} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.44430 ± 0.00074} & \multicolumn{1}{c|}{0.80732 ± 0.00080} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{10} & 31m x 22 \\
\multicolumn{1}{c|}{2017} & \multicolumn{1}{c|}{DeepFM} & 0.4445 & \multicolumn{1}{c|}{0.8085} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.43779 ± 0.00005} & \multicolumn{1}{c|}{0.81407 ± 0.00007} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{128} & 18m x 9 \\
\multicolumn{1}{c|}{2017} & \multicolumn{1}{c|}{DCN} & 0.4419 & \multicolumn{1}{c|}{0.8067} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.43783 ± 0.00017} & \multicolumn{1}{c|}{0.81407 ± 0.00012} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{544} & 14m x 9 \\
\multicolumn{1}{c|}{2018} & \multicolumn{1}{c|}{FwFM} & — & \multicolumn{1}{c|}{—} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.44189 ± 0.00009} & \multicolumn{1}{c|}{0.80985 ± 0.00010} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{14} & 19m x 1 \\
\multicolumn{1}{c|}{2018} & \multicolumn{1}{c|}{xDeepFM} & 0.4418 & \multicolumn{1}{c|}{0.8091} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\textbf{0.43776 ± 0.00019}} & \multicolumn{1}{c|}{\textbf{0.81426 ± 0.00020}} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{156} & 1h9m x 8 \\
\multicolumn{1}{c|}{2019} & \multicolumn{1}{c|}{HFM+} & — & \multicolumn{1}{c|}{—} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.43911} & \multicolumn{1}{c|}{0.81271} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{74} & 1h14m x 3 \\
\multicolumn{1}{c|}{2019} & \multicolumn{1}{c|}{FGCNN} & — & \multicolumn{1}{c|}{—} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.43814 ± 0.00021} & \multicolumn{1}{c|}{0.81418 ± 0.00031} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{87} & 3h9m x 6 \\
\multicolumn{1}{c|}{2019} & \multicolumn{1}{c|}{AutoInt+} & 0.4434 & \multicolumn{1}{c|}{0.8083} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.44148 ± 0.00002} & \multicolumn{1}{c|}{0.81018 ± 0.00004} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{72} & 16m x 1 \\
\multicolumn{1}{c|}{2019} & \multicolumn{1}{c|}{FiGNN} & 0.4411 & \multicolumn{1}{c|}{0.8082} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.43781 ± 0.00010} & \multicolumn{1}{c|}{0.81410 ± 0.00007} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{40} & 1h40m x 14 \\
\multicolumn{1}{c|}{2019} & \multicolumn{1}{c|}{ONN} & {\ul 0.43577} & \multicolumn{1}{c|}{0.8123} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.43805 ± 0.00016} & \multicolumn{1}{c|}{0.81415 ± 0.00027} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{108} & 2h13m x 8 \\
\multicolumn{1}{c|}{2019} & \multicolumn{1}{c|}{FiBiNET} & 0.4423 & \multicolumn{1}{c|}{0.8103} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.43857 ± 0.00021} & \multicolumn{1}{c|}{0.81335 ± 0.00008} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{78} & 2h21m x2 \\
\multicolumn{1}{c|}{2020} & \multicolumn{1}{c|}{LorentzFM} & — & \multicolumn{1}{c|}{—} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.44132} & \multicolumn{1}{c|}{0.81055} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{8} & 2h12m x 20 \\
\multicolumn{1}{c|}{2020} & \multicolumn{1}{c|}{AFN+} & 0.4451 & \multicolumn{1}{c|}{0.8074} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.43865 ± 0.00015} & \multicolumn{1}{c|}{0.81336 ± 0.00007} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{114} & 38m x 6 \\ \hline
\multicolumn{11}{c}{} \\ \hline
\multicolumn{11}{c}{\textbf{Avazu}} \\ \hline
\multicolumn{2}{c|}{} & \multicolumn{2}{c|}{Best Reported} & \multicolumn{2}{c|}{Reproduced} & \multicolumn{4}{c|}{Retuned} & Training \\ \hline
Year & \multicolumn{1}{c|}{Model} & Logloss & \multicolumn{1}{c|}{AUC} & Logloss & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{Logloss} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{\#Params} & \multicolumn{1}{c|}{\#Runs} & Time x Epochs \\ \hline
— & \multicolumn{1}{c|}{LR} & 0.3868 & \multicolumn{1}{c|}{0.7676} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.37991 ± 0.00001} & \multicolumn{1}{c|}{0.78048 ± 0.00006} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{90} & 5m x 26 \\
2010 & \multicolumn{1}{c|}{FM} & 0.3740 & \multicolumn{1}{c|}{0.7793} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.37363 ± 0.00011} & \multicolumn{1}{c|}{0.79079 ± 0.00018} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{187} & 18m x 1 \\
2015 & \multicolumn{1}{c|}{CCPM} & 0.3800 & \multicolumn{1}{c|}{0.7812} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.37183 ± 0.00045} & \multicolumn{1}{c|}{0.79355 ± 0.00072} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{24} & 57m x 1 \\
2016 & \multicolumn{1}{c|}{HOFM} & 0.3756 & \multicolumn{1}{c|}{0.7701} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.37351 ± 0.00011} & \multicolumn{1}{c|}{0.79131 ± 0.00029} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{19} & 1h47m x 1 \\
2016 & \multicolumn{1}{c|}{FFM} & 0.3781 & \multicolumn{1}{c|}{0.7831} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.37114 ± 0.00022} & \multicolumn{1}{c|}{0.79484 ± 0.00044} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{32} & 1h54m x 1 \\
2016 & \multicolumn{1}{c|}{DNN} & — & \multicolumn{1}{c|}{—} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.37048 ± 0.00009} & \multicolumn{1}{c|}{0.79583 ± 0.00008} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{252} & 12m x 1 \\
2016 & \multicolumn{1}{c|}{WideDeep} & 0.3744 & \multicolumn{1}{c|}{0.7749} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.37034 ± 0.00004} & \multicolumn{1}{c|}{0.79575 ± 0.00006} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{52} & 14m x 1 \\
2016 & \multicolumn{1}{c|}{IPNN} & 0.3737 & \multicolumn{1}{c|}{0.7868} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.36839 ± 0.00005} & \multicolumn{1}{c|}{0.79885 ± 0.00007} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{36} & 11m x 1 \\
2016 & \multicolumn{1}{c|}{DeepCross} & 0.3889 & \multicolumn{1}{c|}{0.7643} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.37002 ± 0.00008} & \multicolumn{1}{c|}{0.79620 ± 0.00010} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{45} & 12m x 1 \\
2017 & \multicolumn{1}{c|}{NFM} & 0.3761 & \multicolumn{1}{c|}{0.7708} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.37146 ± 0.00005} & \multicolumn{1}{c|}{0.79399 ± 0.00006} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{54} & 16m x 1 \\
2017 & \multicolumn{1}{c|}{AFM} & 0.3766 & \multicolumn{1}{c|}{0.7740} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.37809 ± 0.00067} & \multicolumn{1}{c|}{0.78403 ± 0.00129} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{67} & 20m x 2 \\
2017 & \multicolumn{1}{c|}{DeepFM} & 0.3742 & \multicolumn{1}{c|}{0.7836} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.37002 ± 0.00005} & \multicolumn{1}{c|}{0.79645 ± 0.00011} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{176} & 21m x 1 \\
2017 & \multicolumn{1}{c|}{DCN} & 0.3721 & \multicolumn{1}{c|}{0.7681} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.36993 ± 0.00013} & \multicolumn{1}{c|}{0.79652 ± 0.00011} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{496} & 7m x 1 \\
2018 & \multicolumn{1}{c|}{FwFM} & 0.3988 & \multicolumn{1}{c|}{0.7406} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.37240 ± 0.00024} & \multicolumn{1}{c|}{0.79253 ± 0.00035} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{15} & 11m x 1 \\
2018 & \multicolumn{1}{c|}{xDeepFM} & 0.3737 & \multicolumn{1}{c|}{0.7855} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.36987 ± 0.00013} & \multicolumn{1}{c|}{0.79650 ± 0.00024} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{72} & 31m x 1 \\
2019 & \multicolumn{1}{c|}{HFM+} & — & \multicolumn{1}{c|}{—} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.36923 ± 0.00004} & \multicolumn{1}{c|}{0.79787 ± 0.00003} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{92} & 43m x 1 \\
2019 & \multicolumn{1}{c|}{FGCNN} & 0.3746 & \multicolumn{1}{c|}{0.7883} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.36961 ± 0.00018} & \multicolumn{1}{c|}{0.79705 ± 0.00027} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{84} & 2h10m x 1 \\
2019 & \multicolumn{1}{c|}{AutoInt+} & 0.3811 & \multicolumn{1}{c|}{0.7774} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.37031 ± 0.00017} & \multicolumn{1}{c|}{0.79587 ± 0.00007} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{75} & 15m x 1 \\
2019 & \multicolumn{1}{c|}{FiGNN} & 0.3817 & \multicolumn{1}{c|}{{\ul 0.8120}} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.37113 ± 0.00009} & \multicolumn{1}{c|}{0.79442 ± 0.00014} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{64} & 2h25m x 1 \\
2019 & \multicolumn{1}{c|}{ONN} & 0.3945 & \multicolumn{1}{c|}{0.7513} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.36767 ± 0.00041} & \multicolumn{1}{c|}{0.80012 ± 0.00009} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{120} & 1h52 x 1 \\
2019 & \multicolumn{1}{c|}{FiBiNET} & 0.3786 & \multicolumn{1}{c|}{0.7832} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\textbf{0.36714 ± 0.00024}} & \multicolumn{1}{c|}{\textbf{0.80088 ± 0.00030}} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{54} & 36m x 1 \\
2020 & \multicolumn{1}{c|}{LorentzFM} & 0.3828 & \multicolumn{1}{c|}{0.7775} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.37417 ± 0.00092} & \multicolumn{1}{c|}{0.79122 ± 0.00199} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{9} & 46m x 17 \\
2020 & \multicolumn{1}{c|}{AFN+} & 0.3718 & \multicolumn{1}{c|}{0.7555} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{0.37061 ± 0.00017} & \multicolumn{1}{c|}{0.79561 ± 0.00029} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{190} & 35m x 1 \\ \hline
\end{tabular}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{FuxiCTR Benchmarks}\label{sec:exp}
In this section, we conduct extensive experiments to evaluate the KD framework for CTR prediction.
% \begin{itemize} 
% \setlength{\itemindent}{0.5ex}
% \setlength{\itemsep}{0.5ex}  
% \item[\textit{RQ1}:] Which is the best KD scheme for CTR prediction?
% \item[\textit{RQ2}:] How dose the unified student model perform compared to the state-of-the-art CTR models?
% \item[\textit{RQ3}:] What are the best model sizes of the teacher and the student models?
% \item[\textit{RQ4}:] What are the impacts of the KD hyper-parameters on student model performance?
% \end{itemize}

\subsection{Experiment Setup}
\subsubsection{Datasets} 
We use three real-world datasets in our experiments: Criteo\footnote{https://www.kaggle.com/c/criteo-display-ad-challenge}, Avazu\footnote{https://www.kaggle.com/c/avazu-ctr-prediction}, and CompanyX (anonymized). The first two are open benchmark datasets released by two leading ad companies, which have been widely used in the previous work (e.g.,~\cite{DeepFM, DCN, xDeepFM, autoint}). The last one is the private dataset from our production recommender system. %All these datasets are collected or sampled from real-world click logs in industry, making the experimental results meaningful to industrial applications. 
Table \ref{tab:Data Statis} summarizes the data statistical information. 


%Besides, they both have tens of millions of samples to train a deep learning CTR prediction model. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[!t]
\small
\centering
\caption{Dataset statistics}\label{tab:Data Statis} 
\begin{tabular}{c||c|c|c|c}
\hline
{Dataset}& \#Instances & \#Fields & \#Features & Positive Ratio \\
\hline 
 Criteo  & 46M & 39 & 1M & 26\% \\
\hline
  Avazu & 40M & 22 & 972K & 17\% \\
\hline
  CompanyX & 231M & 29 & 160K & 5\% \\
\hline
\end{tabular}
% \vspace{-2ex}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 

%% Introduce Criteo and its preparation
\textbf{Criteo}. The Criteo dataset consists of ad click data over a week. It comprises 26 categorical feature fields and 13 numerical feature fields. Following Google's work on DCN~\cite{DCN}, we randomly split the data of the last two days into a validation set and a test set of equal size (6,042,135 samples), while the rest is used for training.

%% Introduce Avazu and its preparation
\textbf{Avazu}. Avazu contains 10 days of click logs. It has a total of 22 fields with categorical features such as app id, app category, device id, etc. Note that we remove the sample\_id field that is useless for CTR prediction. Following the recent work in~\cite{autoint}, we randomly split the dataset into 8:1:1 as the training set, validation set, and test set, respectively.

For the two open datasets, we preprocess the data following the work in~\cite{autoint}: First, we replace the infrequent features (less than a threshold) with a default ``<UNK>'' feature, where the threshold is set to 10 and 5 for Criteo and Avazu, respectively. Second, numerical values in Criteo are normalized to avoid large variance by transforming each value $x$ to $\log^2(x)$, if $x > 2$.

\subsubsection{Evaluation Metrics} 
We employ two widely-used metrics, AUC (Area Under the ROC Curve) and logloss (binary cross-entropy), to evaluate the performance of a CTR prediction model.

% \textbf{AUC} is the Area Under the ROC Curve, a common metric to measure the probability that a randomly chosen positive sample is ranked higher than a randomly chosen negative sample. Higher AUC indicates better CTR prediction performance.

% \textbf{Logloss} can be defined as
% $Logloss = -\frac{1}{N}\sum^{N}_{i}y_i\log p_i$, where $N$ is the number of data samples, $y_i$ is the groundtruth of user clicks ($0$~or $1$) and $p_i$ is the prediction of the evaluated predictor. Lower logloss indicates better CTR prediction performance.

% When considering a large user base as in Criteo and Avazu, a small improvement in prediction accuracy may potentially lead to a large increase in a company's revenue~\cite{DCN}. \textbf{An improvement of 0.001 in logloss or AUC in these datasets is generally considered as practically significant~\cite{autoint}.} 

It is worth noting that an improvement of AUC or logloss at
1\textperthousand ~level is generally considered as practically significant for an industrial CTR prediction problem. This fact has been endorsed by several existing studies from Google~\cite{WideDeep,DeepFM,DCN}, Microsoft~\cite{EnsembleBing}, and Huawei~\cite{DeepFM}. To test statistical significance, we repeat the experiments (in Section~\ref{sec:RQ4}) 10 times by changing the random seed for our student model and the best baseline model, and run the two-tailed paired t-test.

\subsubsection{Implementation Details} 
All models mentioned above are implemented in PyTorch. Each categorical feature is embedded as a feature vector of length 20, 40, and 40 for Criteo, Avazu, and CompanyX, respectively. We empirically set the batch size to 2000 for all models. We apply grid search to find other hype-parameters. We utilize $L_2$ regularization on the feature embeddings and search the regularization weight in the range of $[0, 1e-6, 1e-5, 1e-4, 1e-3]$. We also apply dropout to hidden layers of DNN with dropout rates selected in $[0.1, 0.2, 0.3, 0.4, 0.5]$. The number of hidden layers is in $[2, 3, 4, 5, 6]$. We keep the size of each layer the same and select from $[300, 400, 500, 600]$. Especially, the layers for the crossing layer (in DCN) and CIN (in xDeepFM) vary among $[1,2,3,4]$. As for KD by soft labels, we set $\gamma + \beta=1$ and tune $\beta$ from $0$ to $1$ with a step $0.1$. For KD by hint regression, we set $\gamma=1$ and tune $\beta$ in the range $[0, 1e-6, 1e-5, 1e-4, 1e-3]$. We also try multiple values among $[1,2,3,4,5,7,10,15]$ for temperature $\tau$. Finally, we use Adam~\cite{adam} to optimize all models, and the learning rate is set to the default value 0.001. To avoid overfitting, early stop is used when the metrics on the validation set continuously get worse in three epochs. 


\subsection{Results Analysis}\label{sec:RQ1}
% What we do
%In the next section, we intend to empirically evaluate the performance of different KD schemes for CTR prediction and find the best solution. 

In this section, we aim to study the research question of which KD scheme performs the best for CTR prediction. Here, we define the candidate KD scheme as a combination of the KD strategies (soft label v.s. hint regression) and training methods (pre-train v.s. co-train). Specifically, we use three most representative deep models, including DeepFM, DCN, and xDeepFM, as teacher models. Each model is tuned to its best performance for both Avazu and Criteo. To study the effect of KD schemes only, in this experiment, we fix the size of the student DNN model as $500\times5$. We tune the hyper-parameters for KD via grid search, i.e. $\gamma$ and $\beta$ in Equation~\ref{equ:sum-student} and the temperature $\tau$ in Equation~\ref{equ:softlabel}. 

Table~\ref{sec4-2} shows the performance of the student model DNN under different KD schemes. Especially, the first row indicates the student-only performance, i.e., training the DNN directly. We can make the following observations from the results: 
1) All student models trained via different KD schemes consistently outperform the student-only DNN by a large margin. 
2) The KD scheme of "soft label + pre-train" performs the best among all candidate KD schemes, which indicates that a pretrained teacher model can provide better knowledge guidance from a global view compared with co-train. Moreover, KD via soft label could allow better flexibility than hint regression that strictly limit the inner behaivour of deep models.
In the following experiments, we will mainly consider the "soft label + pre-train" scheme because of its superiority. 





%our teacher and student models all have different architectures. This may yield a hint vector that is difficult to learn via a vanilla DNN. So, hint regression falls behind soft label a bit. 



% Why pretrain good
%A possible explanation for ``pretrain'' beating ``co-train'' is that the training paths of the student model and the teacher model are not necessarily similar due to their different model structures. Thus student models may learn better along an individual path in the ``pretrain'' scheme. On the other hand, ``hint'' seems to contain more information than ``soft label'' since the hint vector is dense and of a larger length. However, the ``soft label'' is demonstrated to be more effective. The possible reasons are twofold: First, the architectures of the teacher model and student model are different, which makes it difficult for the student model to accurately mimic the hint vector; Second, the hint regression requires a learnable regressor for length matching, which may introduce noise and lead to the loss of information. Note that it is possible to match the hint length without the need of the regressor by carefully designing the teacher model and student model. However, it is not practical since the structure of the model is strictly limited in this way.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[!t]
  \centering
  \caption{Performance of different KD schemes. T$\rightarrow$S indicates that T is a teacher and S is a student.}
  \label{sec4-2}
  \includegraphics[width=0.48\textwidth]{fig//Sec42.pdf}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[hbt!]
  \centering
  \caption{Performance across different teacher and student models. Each column represents a teacher model (T) and each row represents a student model (S). 3T denotes an ensemble of teachers: DeepFM + DCN + xDeepFM. The row "w/o KD" represents the performance of using teachers only. LL is short for logloss. The best results in each column are marked in bold.}
  \label{sec4-3}
  \includegraphics[width=1\textwidth]{fig//Sec4-3.pdf}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sections2/3_approach.tex <==
\section{TagGNN Approach}\label{sec:approach}
In this section, we first introduce the motivation of our model design, and then present the architecture of our TagGNN framework. We show how it is trained and used for item tagging problem. 

\subsection{Motivation and Overview}

Traditional approaches for solving item tagging problem is to treat it as a multi-label text classification problem. We can train $N$ classifiers for each tag to determine which tags belong to the item. Although this approach is simple and fast, it has the following limitations that hinder the improvement of accuracy.

Firstly, the information between items and tags is not well utilized. In the naive multi-label classification approach, each training sample <item, tag> is used individually, and there is no direct feature interaction between items and tags, leading to unsatisfactory prediction accuracy.

Secondly, it neglects the semantic relationships between tags. For example, as shown in Figure~\ref{fig:app_demo}, Pokemon has two strongly correlated tags, i.e., AR (Augmented Reality) and VR (Virtual Reality). These two techniques are often applied in the same product and thus often appear together. Relationships between tags are especially useful for tag complement task (which means we have known the item's partial tags and want to predict the other tags), since one tag may indicate the strong existence or non-existence for its relative or opposite tags.    

Thirdly, query information, which is crucial in IR, has not been fully exploited for item tagging. In fact, users' queries for finding the item, to a great extent indicates the properties of this item. For example, it is probable that a user downloads ``Facebook'' application under the query ``chat''. Query ``chat'' can imply tags like ``chat'', ``social'' and ``video'' which is suitable for ``Facebook'' application. How to effectively utilize users' large amount of query information is an very important part to build a more accurate tagging system.  

To solve the above 3 limitations, we model the item tagging problem from the view of graph, and propose TagGNN framework to learn better representation of the query, item and tag, so as to obtain more satisfactory tagging performance.


\begin{figure*}[htbp]
    \begin{center}
    %\framebox[4.0in]{$\;$}
    % \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
    \includegraphics[width = 1\linewidth]{fig2/TagGNN-1.png}
    \end{center}
    \vspace{-2ex}
    \caption{Overview of TagGNN}
    \label{TagGNN}
\end{figure*}


\subsection{Model Overview}
Figure~\ref{TagGNN} shows an overview of TagGNN. Suppose that we have got the related queries of the items from the IR system, and we also know the items' corresponding tags. Then we build an undirected  tripartite graph to link query, item and tag together. This heterogeneous tripartite graph has three types of nodes, i.e., query, item and tag, and two types of edges commonly, i.e., query-item and item-tag. The edge can represent different meanings depending on different real scenarios. For example, in the App Store scenario (app tagging),  the query-item edge can represent the click or download of the app under the query. Note that the item node can be unilateral or complete isolated if we do not know any related queries or existing tags (or both) of the item. Then, we employ a GNN tailored for item tagging to propagate all of the information in the graph to get better item and tag representation. Finally, 
we calculate the similarity between the item representation and  all tags representation and choose $K$ tags with the highest similarities as the our top$K$ prediction. 
In the following, we elaborate every part of our TagGNN framework.

\subsection{Initial Representation}
\label{initial representation}
We choose the query content, the item name and the tag name as the initial features of the query, item and tag nodes respectively. Without loss of generality, suppose that the node contains a string of words (content, name, description or others) $(w_1, w_2,..., w_n)$, we can use any models that can deal with the sequence, such as RNN and CNN, to get the initial representation $h$ of the node. 
In particular, since the tag sets are fixed, we add an extra id embedding, which is a one-hot vector, for each tag node. For simplicity, here we just average all of word embeddings as the initial representation:  
\begin{equation}
h = \left\{
             \begin{array}{lr}
              \frac{1}{n}\sum_{i=1}^{n}{w_i},\ \, \text{if\,query\,or\,item\,node}
             \\
              \frac{1}{n}\sum_{i=1}^{n}{w_i} + id,\ \, \text{if\,tag\,node}&  
             \end{array}
\right.
\end{equation}
where $id$ is the one-hot id embedding for the tag node.

As for the edge, if it has a weight, e.g., the click times of the app under the query for query-item edge, we can use the weight to enhance the message passing through this edge by simply multiply the message representation with the weight scalar. If the weight range is very large, we can use some feature scaling strategies like min-max normalization or standar`qdization to rescale. Besides, we can also perform feature discretization, e.g., binning~\cite{zheng2018feature} , to get the initial edge representation.
If the edge not has weight, we just set all edges' weights to 1.

\subsection{Learning process of TagGNN}
In this part, we first give a brief review of GNN and then detail the feature learning process of TagGNN that is tailored for item tagging.

\subsubsection{GNN Recap}
Suppose that a graph $G$ has the initial node representation $h_v$ for each node $v$ and edge representation $e_{vw}$ for each edge $v$->$w$, a typical one-layer GNN can learn new representation by the following message passing paradigm described in \cite{gilmer2017neural}:
\begin{eqnarray}
  \bm{m}_{v}&=&\sum_{w \in \mathcal{N}(v)} M\left(\bm{h}_{v},\bm{h}_{w}, \bm{e}_{v w}\right),\\
  \bm{h}^{new}_{v}&=&U\left(\bm{h}_{v}, \bm{m}_{v}\right),
\end{eqnarray}
where $\mathcal{N}(v)$ denotes the neighbors of node $v$ in graph $G$,  $M$ is the message function that is responsible for collecting information from neighbors, and $U$ is the update function for fusing collected information ${m}_v$ with old node representation ${h}_v$ to obtain the new node representation ${h}^{new}_{v}$.

\subsubsection{TagGNN Propagation}
TagGNN also follows the message passing paradigm. When a node aggregating its neighbors' information, it first calculates the similarity with each neighbor based on their semantic (node) representation and  relationship (edge) representation.
Then it aggregates all of neighbor's representation by the similarity weights to form the message representation.
Formally, as mentioned in~\ref{initial representation}, if the edge representation $e_{vw}$ is a vector, the similarity is:
\begin{equation}
   \alpha_{vw}=\frac{\exp \left(\operatorname{LeakyReLU}\left(\mathbf{a}^{T}\left[\bm{W} \bm{h}_{v} \| \bm{W} \bm{h}_{w} \| \bm{e}_{vw}\right]\right)\right)}{\sum_{k \in \mathcal{N}_{v}} \exp \left(\operatorname{LeakyReLU}\left(\mathbf{a}^{T}\left[\bm{W} \bm{h}_{v} \| \bm{W} \bm{h}_{k} \| \bm{e}_{vk}\right]\right)\right)},
\end{equation}
While if the edge representation $e_{vw}$ is a scalar, the similarity is:
\begin{equation}
   \alpha_{vw}=e_{vw} \times \frac{\exp \left(\operatorname{LeakyReLU}\left(\mathbf{a}^{T}\left[\bm{W} \bm{h}_{v} \| \bm{W} \bm{h}_{w}\right]\right)\right)}{\sum_{k \in \mathcal{N}_{v}} \exp \left(\operatorname{LeakyReLU}\left(\mathbf{a}^{T}\left[\bm{W} \bm{h}_{v} \| \bm{W} \bm{h}_{k}\right]\right)\right)},
\end{equation}
The message function $M$ is:
\begin{equation}
   \bm{h}_{m}=\sum_{w \in \mathcal{N}_{v}} \alpha_{v w} \bm{W} \bm{h}_{w},
\end{equation}
where $W \in \mathbb{R}^{D}$ is a transformation matrix to transform the node into a new feature space, $\mathbf{a}$ is a global context vector to determine the similarity between the two nodes. 

With the help of this attention mechanism, the node can put more reasonable weights to its neighbors so that it can distinguish which neighbors have significant information while which neighbors may be just ``noise'' that should be ignored. 

Then, in order to generate new powerful node representation, different types of nodes have different transformation matrices to map the original representation and its coming message representation into a new unified space so that they can be merged. In practice, we stack $N$ such GNN layers to capture higher-order neighbors' information. However, GNN often faces the over-smoothing problem~\cite{rong2019dropedge} as the number of layers get deeper. To mitigate this and obtain more comprehensive representations, we adopt a gated skip-connection mechanism。
Formally, the update function $U$ is:
\begin{eqnarray}
    \hat{h}_{type} = \sigma(W_{type}(h_{type} + h_m)),\\
    z = \operatorname{sigmoid}(U_1\hat{h}_{type} + U_2h_{type} + b),\\
    h_{type}^{new} = z \odot \hat{h}_{type} + (1 - z) \odot h
\end{eqnarray}
where $W_{type}$ can be 3 different transformation matrices for query, item and tag nodes respectively, $U_1$, $U_2$, $b$ are trainable parameters. $z$ controls the proportion of the original representation and the new learned representation to get the final new representation.

\subsection{Training and Inference}
\label{training}
From the perspective of graph, we deem the item tagging problem as a link prediction problem, i.e., to predict which tag nodes should be linked to the target item node.

In the training phase, we compute dot-product similarity between the learned item representation and tag representation, and compute its binary cross-entropy loss $\bm{Loss_1}$ with the ground truth (0 or 1 represents link or not link).
Moreover, note that there may be some isolated item nodes in the graph. For the isolated node, we do not know any existing query or tag information about it, and we stipulate that its representation will not be updated by TagGNN propagation. Therefore, to empower TagGNN with the ability to handle this cold start problem, we also compute dot-product similarity between the initial item representation and learned tag representation (note that tag nodes cannot be isolated), and compute its binary cross-entropy loss $\bm{Loss_2}$ with the ground truth. Finally we optimize the model by reducing these two losses with stochastic gradient descent algorithms.Formally, 
\begin{eqnarray}
    &&
    Loss_1 = BCE(y, \  h_{item}^{new} \cdot h_{tag}^{new}), \\
    &&
    Loss_2 = BCE(y, \  h_{item} \cdot h_{tag}^{new}), \\ 
    &&
    Loss = Loss1 + \gamma Loss2
\end{eqnarray}
where $BCE$ is binary cross-entropy loss, $y$ is the ground truth for the edge between the item node and the tag node. $\gamma$ is the hyper-parameter to adjust the proportion of $Loss_1$ and $Loss_2$. 

When Inference, since the model has been optimized to be able to deal with isolated item nodes. we do not distinguish whether the target item node is isolated or not. We just compute similarities between the target item representation and all of tags representation after TagGNN propagation, and choose $K$ tags with the highest similarity as our prediction result. 


\subsection{Model Strengths}
Compared with the traditional multi-label text classification approaches, our TagGNN can effectively improve the item tagging performance from the following perspectives.

Firstly, under our TagGNN framework, items and tags can have direct interactions since they are neighbors in the graph. Thanks to deeper semantic interactions in the propagation of TagGNN, their learned representation becomes more powerful. 

Secondly, relationships between tags are effectively utilized. Since the item node aggregates its neighbor tag nodes, its new learned representation will contain the tags information. Therefore, when we compute the similarity between items and tags, the semantic relationships between tags also play a role. Besides, if we use multi-layer GNN, there will be indirect interactions between tags and tags, potentially improving the quality of learned semantic representation.

Thirdly, query information is successfully included in our framework to bring improvement. By enhancing the item with the queries' features, the item's semantic representation becomes more rich and representative, which can greatly help to find the related tags. 

Moreover, as shown in Figure~\ref{TagGNN}, you can also view TagGNN, a tripartite graph framework, from the perspective of two bipartite graphs, i.e., query-item graph (TagGNN-QI) and item-tag graph (TagGNN-IT). We experimentally demonstrate that these two simplified variants also have good promotion compared with other baselines. You can flexibly choose the most suitable model in practice.
